Descent Before Hardness: Orbit-Gap Obstructions in Exact Certification

Tractability tests are often computed from input syntax: support-graph treewidth, local coefficient patterns, backdoor tests, or action-count bounds. Before such a test can be lower-bounded or made algorithmic, it must define a predicate on the exact-certification problem itself. Equivalent presentations must receive the same verdict. The semantic object is the correctness quotient, whose classes are states with the same correct outputs. Correctness-preserving presentation moves generate closure orbits. A target that changes inside one closure orbit has an orbit gap and fails descent. Exact closure-invariant classification is possible exactly when the positive and negative orbit hulls are disjoint; the positive hull is then the least exact classifier, and computable orbit representatives make the classifier algorithmic. The results separate three layers. The descent layer gives orbit-gap obstructions for raw local syntax, raw action and coordinate counts, and raw support-graph predicates. The post-descent complexity layer applies ordinary reductions to descended objects: graph-predicate lower bounds transfer through action-gap graph extraction, and Action-Gap-Treewidth is NP-complete when the width bound is part of the input. The certification layer asks whether a proxy descends: for split proxies $b\wedge\varphi(z)$, SAT reduces to non-descent and UNSAT reduces to descent. Positive regimes use quotient-preserving normalizations or catalogues before model checking; bounded quotient size, bounded full Gaifman treewidth of the constructed quotient, sparse unary-gap certificates, and strict-margin perturbation balls give explicit cost bounds after quotient construction.

==> content/assumption_ledger_auto.tex <==
% Auto-generated by scripts/build_papers.py. No assumption ledger source found.


==> content/proof_hardness_index_auto.tex <==
% Auto-generated by scripts/build_papers.py. Do not edit manually.
% Generated: 2026-07-01T12:55:36.406145
% Manuscript: paper4d
\begingroup
\scriptsize
\sloppy
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}
\begin{longtable}{@{}>{\raggedright\arraybackslash}m{0.19\linewidth}>{\raggedright\arraybackslash}m{0.13\linewidth}>{\raggedright\arraybackslash}m{0.26\linewidth}>{\raggedright\arraybackslash}m{0.38\linewidth}@{}}
\toprule
\textbf{Manuscript handle} & \textbf{Hardness profile} & \textbf{Regime tags} & \textbf{Lean support} \\
\midrule
\endfirsthead
\toprule
\textbf{Manuscript handle} & \textbf{Hardness profile} & \textbf{Regime tags} & \textbf{Lean support} \\
\midrule
\endhead
\endfoot
\bottomrule
\endlastfoot
\nolinkurl{thm:action-gap-treewidth-np-complete} & \nolinkurl{NP-complete} & - & \LH{FR394}, \LH{FR395}, \LH{FR396} \\
\midrule
\nolinkurl{cor:boolean-payload-transfer} & \nolinkurl{structural/exact} & - & \LH{FR223}, \LH{FR224}, \LH{FR225}, \LH{FR226}, \LH{FR227}, \LH{FR228}, \LH{FR229}, \LH{FR230}, \LH{FR231}, \LH{FR340}, \LH{FR341} \\
\midrule
\nolinkurl{cor:catalogue-classifiers-compositional} & \nolinkurl{structural/exact} & - & \LH{FR384}, \LH{FR385}, \LH{FR386}, \LH{FR387}, \LH{FR388}, \LH{FR389} \\
\midrule
\nolinkurl{cor:correctness-quotient-universality} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{cor:domain-restriction-only-removes-orbit-gaps} & \nolinkurl{structural/exact} & - & \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256} \\
\midrule
\nolinkurl{cor:every-state-equivalence-relation-is-realizable-as-exact-output-semantics} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{cor:full-binary-pairwise-no-go} & \nolinkurl{structural/exact} & - & \LH{FR350} \\
\midrule
\nolinkurl{cor:least-exact-classifier} & \nolinkurl{structural/exact} & - & \LH{FR358} \\
\midrule
\nolinkurl{cor:named-guarantee-semantics-transfer} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{cor:no-correct-tractability-classifier} & \nolinkurl{structural/exact} & - & \LH{FR193}, \LH{FR197}, \LH{FR198}, \LH{FR199} \\
\midrule
\nolinkurl{cor:orbit-gap-completeness-domain} & \nolinkurl{structural/exact} & - & \LH{FR201}, \LH{FR202}, \LH{FR203}, \LH{FR204}, \LH{FR210}, \LH{FR211}, \LH{FR212}, \LH{FR213}, \LH{FR367}, \LH{FR368}, \LH{FR369}, \LH{FR370}, \LH{FR371}, \LH{FR372}, \LH{FR373}, \LH{FR374}, \LH{FR375} \\
\midrule
\nolinkurl{cor:orbit-gap-template} & \nolinkurl{structural/exact} & - & \LH{FR185} \\
\midrule
\nolinkurl{cor:predicate-transfer} & \nolinkurl{structural/exact} & - & \LH{FR223}, \LH{FR224}, \LH{FR225}, \LH{FR226}, \LH{FR227}, \LH{FR228}, \LH{FR229}, \LH{FR230}, \LH{FR231}, \LH{FR340}, \LH{FR341} \\
\midrule
\nolinkurl{cor:relational-output-transfer} & \nolinkurl{structural/exact} & - & \LH{FR223}, \LH{FR224}, \LH{FR225}, \LH{FR226}, \LH{FR227}, \LH{FR228}, \LH{FR229}, \LH{FR230}, \LH{FR231}, \LH{FR340}, \LH{FR341} \\
\midrule
\nolinkurl{cor:set-valued-payload-transfer} & \nolinkurl{structural/exact} & - & \LH{FR223}, \LH{FR224}, \LH{FR225}, \LH{FR226}, \LH{FR227}, \LH{FR228}, \LH{FR229}, \LH{FR230}, \LH{FR231}, \LH{FR340}, \LH{FR341} \\
\midrule
\nolinkurl{cor:small-uniform-perturbations-can-flip-relevance} & \nolinkurl{structural/exact} & - & \LH{FR264}, \LH{FR267} \\
\midrule
\nolinkurl{cor:small-uniform-perturbations-can-flip-sufficiency} & \nolinkurl{structural/exact} & - & \LH{FR264}, \LH{FR267} \\
\midrule
\nolinkurl{cor:strict-margin-quotient-mso-stability} & \nolinkurl{structural/exact} & - & \LH{FR476}, \LH{FR477}, \LH{FR478} \\
\midrule
\nolinkurl{cor:totalized-set-valued-payload-transfer} & \nolinkurl{structural/exact} & - & \LH{FR223}, \LH{FR224}, \LH{FR225}, \LH{FR226}, \LH{FR227}, \LH{FR228}, \LH{FR229}, \LH{FR230}, \LH{FR231}, \LH{FR340}, \LH{FR341} \\
\midrule
\nolinkurl{cor:universal-exact-specification-no-go} & \nolinkurl{structural/exact} & - & \LH{FR351}, \LH{FR361} \\
\midrule
\nolinkurl{cor:universal-scope-rigorously-specified-problems} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{lem:affine-shift-obstruction} & \nolinkurl{structural/exact} & - & \LH{FR15}, \LH{FR16}, \LH{FR17}, \LH{FR18}, \LH{FR19}, \LH{FR20}, \LH{FR185} \\
\midrule
\nolinkurl{lem:closure-law-invariance-iff-orbit-constancy} & \nolinkurl{structural/exact} & - & \LH{FR362} \\
\midrule
\nolinkurl{prop:abstract-fiber-gap-descent} & \nolinkurl{structural/exact} & - & \LH{FR201}, \LH{FR202}, \LH{FR203}, \LH{FR204}, \LH{FR210}, \LH{FR211}, \LH{FR212}, \LH{FR213}, \LH{FR367}, \LH{FR368}, \LH{FR369}, \LH{FR370}, \LH{FR371}, \LH{FR372}, \LH{FR373}, \LH{FR374}, \LH{FR375} \\
\midrule
\nolinkurl{prop:action-gap-treewidth-realizes-graph-treewidth} & \nolinkurl{structural/exact} & - & \LH{FR394}, \LH{FR395}, \LH{FR396} \\
\midrule
\nolinkurl{prop:approximate-relevance-needs-stability-control} & \nolinkurl{structural/exact} & - & \LH{FR263}, \LH{FR266} \\
\midrule
\nolinkurl{prop:closure-operations-preserve-certification} & \nolinkurl{structural/exact} & - & \LH{FR15}, \LH{FR16}, \LH{FR17}, \LH{FR18}, \LH{FR19}, \LH{FR20}, \LH{FR55}, \LH{FR56}, \LH{FR57}, \LH{FR58}, \LH{FR59}, \LH{FR60}, \LH{FR83}, \LH{FR84}, \LH{FR85} \\
\midrule
\nolinkurl{prop:closurehull-fixed-points} & \nolinkurl{structural/exact} & - & \LH{FR355} \\
\midrule
\nolinkurl{prop:countable-specifications-admit-countable-boolean-presentations} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{prop:depends-only-on-opt} & \nolinkurl{structural/exact} & - & \LH{FR30}, \LH{FR31}, \LH{FR32}, \LH{FR33}, \LH{FR34}, \LH{FR35}, \LH{FR37}, \LH{FR51}, \LH{FR176}, \LH{FR177} \\
\midrule
\nolinkurl{prop:distinct-profile-compression} & \nolinkurl{structural/exact} & - & \LH{FR206}, \LH{FR207}, \LH{FR208}, \LH{FR209} \\
\midrule
\nolinkurl{prop:every-exact-specification-admits-coordinate-presentation} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{prop:finite-specifications-admit-coordinate-presentations} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{prop:finite-specifications-admit-low-dimensional-boolean-presentations} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{prop:full-binary-pairwise-domain-closure} & \nolinkurl{structural/exact} & - & \LH{FR348}, \LH{FR349} \\
\midrule
\nolinkurl{prop:global-approximation-stability} & \nolinkurl{structural/exact} & - & \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR300}, \LH{FR301} \\
\midrule
\nolinkurl{prop:minimal-sufficient-canonical} & \nolinkurl{structural/exact} & - & \LH{FR352} \\
\midrule
\nolinkurl{prop:orbit-gap-completeness} & \nolinkurl{structural/exact} & - & \LH{FR201}, \LH{FR202}, \LH{FR203}, \LH{FR204}, \LH{FR210}, \LH{FR211}, \LH{FR212}, \LH{FR213}, \LH{FR367}, \LH{FR368}, \LH{FR369}, \LH{FR370}, \LH{FR371}, \LH{FR372}, \LH{FR373}, \LH{FR374}, \LH{FR375} \\
\midrule
\nolinkurl{prop:semantic-claims-depend-only-on-output-equivalence} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{prop:semantically-extensional-claims-factor-through-the-quotient} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199}, \LH{FR232}, \LH{FR233}, \LH{FR234}, \LH{FR235}, \LH{FR236}, \LH{FR237}, \LH{FR238}, \LH{FR239}, \LH{FR240}, \LH{FR241}, \LH{FR242}, \LH{FR243}, \LH{FR244}, \LH{FR252}, \LH{FR253}, \LH{FR254}, \LH{FR255}, \LH{FR256}, \LH{FR268}, \LH{FR269}, \LH{FR270}, \LH{FR271}, \LH{FR272}, \LH{FR273}, \LH{FR274}, \LH{FR275}, \LH{FR276}, \LH{FR277}, \LH{FR278}, \LH{FR279}, \LH{FR280}, \LH{FR281}, \LH{FR282}, \LH{FR283}, \LH{FR284}, \LH{FR285}, \LH{FR286}, \LH{FR287}, \LH{FR288}, \LH{FR289}, \LH{FR290}, \LH{FR291}, \LH{FR292}, \LH{FR293}, \LH{FR294}, \LH{FR295}, \LH{FR296}, \LH{FR297}, \LH{FR298}, \LH{FR299}, \LH{FR300}, \LH{FR301}, \LH{FR302}, \LH{FR303}, \LH{FR304}, \LH{FR305}, \LH{FR306}, \LH{FR307}, \LH{FR308}, \LH{FR309}, \LH{FR310}, \LH{FR311}, \LH{FR312}, \LH{FR313}, \LH{FR314}, \LH{FR315}, \LH{FR345}, \LH{FR351} \\
\midrule
\nolinkurl{prop:zero-distortion-refines-quotient} & \nolinkurl{structural/exact} & - & \LH{FR30}, \LH{FR31}, \LH{FR32}, \LH{FR33}, \LH{FR34}, \LH{FR35}, \LH{FR37}, \LH{FR51}, \LH{FR176}, \LH{FR177} \\
\midrule
\nolinkurl{thm:bounded-distinct-profile-positive-regime} & \nolinkurl{structural/exact} & - & \LH{FR206}, \LH{FR207}, \LH{FR208}, \LH{FR209} \\
\midrule
\nolinkurl{thm:bounded-quotient-size-mso-tractability} & \nolinkurl{structural/exact} & - & \LH{FR470}, \LH{FR471}, \LH{FR472}, \LH{FR473}, \LH{FR474}, \LH{FR475} \\
\midrule
\nolinkurl{thm:bounded-quotient-treewidth-mso-tractability} & \nolinkurl{structural/exact} & - & \LH{FR460}, \LH{FR461}, \LH{FR462}, \LH{FR463}, \LH{FR464}, \LH{FR465}, \LH{FR466}, \LH{FR467}, \LH{FR468}, \LH{FR469} \\
\midrule
\nolinkurl{thm:closure-sound-package-no-go} & \nolinkurl{structural/exact} & - & \LH{FR193} \\
\midrule
\nolinkurl{thm:correct-classifier-forces-invariance} & \nolinkurl{structural/exact} & - & \LH{FR197}, \LH{FR198}, \LH{FR199} \\
\midrule
\nolinkurl{thm:exact-classification-hull-separation} & \nolinkurl{structural/exact} & - & \LH{FR356}, \LH{FR357} \\
\midrule
\nolinkurl{thm:finite-orbit-catalogue-classifiers} & \nolinkurl{structural/exact} & - & \LH{FR376}, \LH{FR377}, \LH{FR378}, \LH{FR379}, \LH{FR380}, \LH{FR381}, \LH{FR382}, \LH{FR383} \\
\midrule
\nolinkurl{thm:graph-predicate-hardness-transfer} & \nolinkurl{structural/exact} & - & \LH{FR491}, \LH{FR492}, \LH{FR503}, \LH{FR504}, \LH{FR505}, \LH{FR506}, \LH{FR507}, \LH{FR508} \\
\midrule
\nolinkurl{thm:normalized-unary-gap-positive-regime} & \nolinkurl{structural/exact} & - & \LH{FR390}, \LH{FR391}, \LH{FR392}, \LH{FR393} \\
\midrule
\nolinkurl{thm:optimizer-computation-classifier-forces-invariance} & \nolinkurl{structural/exact} & - & \LH{FR248}, \LH{FR259}, \LH{FR260}, \LH{FR261}, \LH{FR262}, \LH{FR316}, \LH{FR317}, \LH{FR318}, \LH{FR319}, \LH{FR320}, \LH{FR321}, \LH{FR322}, \LH{FR323}, \LH{FR324}, \LH{FR325}, \LH{FR326}, \LH{FR327}, \LH{FR328}, \LH{FR329}, \LH{FR330}, \LH{FR331}, \LH{FR332}, \LH{FR333}, \LH{FR334}, \LH{FR335}, \LH{FR336} \\
\midrule
\nolinkurl{thm:post-descent-quotient-mso-evaluation} & \nolinkurl{structural/exact} & - & \LH{FR423}, \LH{FR424}, \LH{FR425}, \LH{FR426}, \LH{FR427}, \LH{FR428}, \LH{FR429}, \LH{FR430}, \LH{FR431}, \LH{FR432}, \LH{FR433}, \LH{FR434}, \LH{FR435}, \LH{FR458}, \LH{FR459} \\
\midrule
\nolinkurl{thm:quotient-flip-graph-realization} & \nolinkurl{structural/exact} & - & \LH{FR411}, \LH{FR412}, \LH{FR413}, \LH{FR414}, \LH{FR415}, \LH{FR416}, \LH{FR417}, \LH{FR418}, \LH{FR419}, \LH{FR420}, \LH{FR421}, \LH{FR422} \\
\midrule
\nolinkurl{thm:raw-action-count-duplication-orbit-gap} & \nolinkurl{structural/exact} & - & \LH{FR406}, \LH{FR407}, \LH{FR408}, \LH{FR409}, \LH{FR410} \\
\midrule
\nolinkurl{thm:raw-coordinate-count-irrelevant-coordinate-orbit-gap} & \nolinkurl{structural/exact} & - & \LH{FR485}, \LH{FR486}, \LH{FR487}, \LH{FR488}, \LH{FR489}, \LH{FR490} \\
\midrule
\nolinkurl{thm:sparse-unary-gap-quotient-pipeline} & \nolinkurl{structural/exact} & - & \LH{FR479}, \LH{FR480}, \LH{FR481}, \LH{FR482}, \LH{FR483}, \LH{FR484} \\
\midrule
\nolinkurl{thm:split-proxy-descent-certification-hardness} & \nolinkurl{structural/exact} & - & \LH{FR491}, \LH{FR492}, \LH{FR493}, \LH{FR494}, \LH{FR495}, \LH{FR496}, \LH{FR497}, \LH{FR498}, \LH{FR499}, \LH{FR500}, \LH{FR501}, \LH{FR502} \\
\bottomrule
\end{longtable}
\endgroup

\noindent\textit{Auto summary: indexed 57 claims by hardness profile (NP-complete=1; structural/exact=56).}


==> lean-handle-macros.tex <==
% Auto-generated by scripts/build_papers.py. Do not edit manually.
% Lean handle macro definitions: compact footnote markers in body text
\providecommand{\LH}[1]{}
\renewcommand{\LH}[1]{\leavevmode\nobreak\hyperlink{lh:#1}{\mbox{\ttfamily\nolinkurl{#1}}}}
\providecommand{\LHrng}[3]{}
\renewcommand{\LHrng}[3]{\leavevmode\nobreak\hyperlink{lh:#1#2}{\mbox{\ttfamily\nolinkurl{#1#2-#3}}}}
\newif\ifleanmetaseen
\leanmetaseenfalse
\makeatletter
\providecommand{\leanmetapendinghandles}{}
\global\let\leanmetapendinghandles\@empty
\providecommand{\leanmetapending}[1]{}
\renewcommand{\leanmetapending}[1]{\def\leanmetatest{#1}\ifx\leanmetatest\@empty\global\let\leanmetapendinghandles\@empty\else\gdef\leanmetapendinghandles{#1}\fi}
\providecommand{\leanmetaproofpendinghandles}{}
\global\let\leanmetaproofpendinghandles\@empty
\providecommand{\leanmetaproofpending}[1]{}
\renewcommand{\leanmetaproofpending}[1]{\def\leanmetatest{#1}\ifx\leanmetatest\@empty\global\let\leanmetaproofpendinghandles\@empty\else\gdef\leanmetaproofpendinghandles{#1}\fi}
\providecommand{\leanmetaheadmark}{}
\renewcommand{\leanmetaheadmark}{\ifx\leanmetapendinghandles\@empty\else\nobreak\hspace{0.2em}\refstepcounter{footnote}\footnotemark[\value{footnote}]\footnotetext[\value{footnote}]{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi\leanmetapendinghandles}\global\let\leanmetapendinghandles\@empty\fi}
\providecommand{\leanmetaproofmark}{}
\renewcommand{\leanmetaproofmark}{\ifx\leanmetaproofpendinghandles\@empty\else\ifhmode\unskip\footnote{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi\leanmetaproofpendinghandles}\else\refstepcounter{footnote}\footnotemark[\value{footnote}]\footnotetext[\value{footnote}]{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi\leanmetaproofpendinghandles}\fi\global\let\leanmetaproofpendinghandles\@empty\fi}
\@ifundefined{newtheoremstyle}{}{\@ifundefined{thmname}{}{%
  \newtheoremstyle{leanplain}
    {6pt}{6pt}{\itshape}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}\leanmetaheadmark}
  \newtheoremstyle{leandefinition}
    {6pt}{6pt}{}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}\leanmetaheadmark}
  \newtheoremstyle{leandef}
    {6pt}{6pt}{}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}\leanmetaheadmark}
  \newtheoremstyle{leanremark}
    {6pt}{6pt}{}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}\leanmetaheadmark}
}}
\makeatother
\providecommand{\leanmeta}[1]{}
\renewcommand{\leanmeta}[1]{\ifhmode\unskip\footnote{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi#1}\else\refstepcounter{footnote}\footnotemark[\value{footnote}]\footnotetext[\value{footnote}]{\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi#1}\fi}


==> paper_title_auto.tex <==
% Auto-generated by scripts/build_papers.py. Canonical manuscript title.
\providecommand{\PaperTitleAuto}{Descent Before Hardness: Orbit-Gap Obstructions in Exact Certification}

